Reassessing the computational advantage of quantum-controlled ordering of gates

Research on indefinite causal structures is a rapidly evolving field that has a potential not only to make a radical revision of the classical understanding of space-time but also to achieve enhanced functionalities of quantum information processing. For example, it is known that indefinite causal structures provide exponential advantage in communication complexity when compared to causal protocols. In quantum computation, such structures can decide whether two unitary gates commute or anticommute with a single call to each gate, which is impossible with conventional (causal) quantum algorithms. A generalization of this effect to $n$ unitary gates, originally introduced in M. Ara\'ujo et al., Phys. Rev. Lett. 113, 250402 (2014) and often called Fourier promise problem (FPP), can be solved with the quantum-$n$-switch and a single call to each gate, while the best known causal algorithm so far calls $O(n^2)$ gates. In this work, we show that this advantage is smaller than expected. In fact, we present a causal algorithm that solves the only known specific FPP with $O(n \log(n))$ queries and a causal algorithm that solves every FPP with $O(n\sqrt{n})$ queries. Besides the interest in such algorithms on their own, our results limit the expected advantage of indefinite causal structures for these problems.

==> circstring2.tex <==
\Qcircuit @C=0.5em @R=1em {
                   &  \vdots    &  &                         &                         &                         &              &                         &                         &                         &     & \vdots &\\\\
\lstick{\ket{c^x_{k_3,j}}} & \text{...} &  & \ctrl{3}                & \qw                     & \qw                     & \qw          & \qw                     & \qw                     & \ctrlo{3}               & \qw & \text{...}            & \rstick{(\omega^{x_{k_3,j}\cdot y})}\\
\lstick{\ket{c^x_{k_2,j}}} & \text{...} &  & \qw                     & \ctrl{2}                & \qw                     & \qw          & \qw                     & \ctrlo{2}               & \qw                     & \qw & \text{...}            &\rstick{(\omega^{x_{k_2,j}\cdot y})}\\
\lstick{\ket{c^x_{k_1,j}}} & \text{...} &  & \qw                     & \qw                     & \ctrl{1}                & \qw          & \ctrlo{1}               & \qw                     & \qw                     & \qw & \text{...}            &\rstick{(\omega^{x_{k_1,j}\cdot y})}\\
\lstick{\ket{\Psi_{j}}}       & \text{...} &  & \gate{U_{k_3}} & \gate{U_{k_2}} & \gate{U_{k_1}} & \gate{U_{k_0}} & \gate{U_{k_1}} & \gate{U_{k_2}} & \gate{U_{k_3}} & \qw & \text{...}&
}

==> circswap.tex <==
\Qcircuit @C=1em @R=1em {
\lstick{\ket{c_{n-1, 1}}}                     & \qw        & \qw &             &  &  &  &  &  &  &  &  &  & \lstick{\ket{c_{n-1, 1}}}                     & \qw            & \qw        & \qw            & \qw \\
\lstick{\vdots}                               &            &     &             &  &  &  &  &  &  &  &  &  & \lstick{\vdots}                               &                &            &                &     \\
                                              &            &     &             &  &  &  &  &  &  &  &  &  &                                               &                &            &                &     \\
\lstick{\ket{c_{k,  i}}}                      & \ctrl{8}   & \qw &             &  &  &  &  &  &  &  &  &  & \lstick{\ket{c_{k,  i}}}                      & \ctrl{8}       & \qw        & \ctrl{8}       & \qw \\
\lstick{\vdots}                               &            &     &             &  &  &  &  &  &  &  &  &  & \lstick{\vdots}                               &                &            &                &     \\
                                              &            &     &             &  &  &  &  &  &  &  &  &  &                                               &                &            &                &     \\
\lstick{\ket{c_{1,  \hat{i}}}}                & \qw        & \qw &             &  &  &  &  &  &  &  &  &  & \lstick{\ket{c_{1,  \hat{i}}}}                & \qw            & \qw        & \qw            & \qw \\
                                              &            &     &             &  &  &  &  &  &  &  &  &  &                                               &                &            &                &     \\
\lstick{\ket{\Psi_{2,1}}}                     & \qw        & \qw &             &  &  &  &  &  &  &  &  &  & \lstick{\ket{\Psi_{2,1}}}                     & \qw            & \qw        & \qw            & \qw \\
\lstick{\vdots}                               &            &     &             &  &  &  &  &  &  &  &  &  & \lstick{\vdots}                               &                &            &                &     \\
                                              &            &     & \Rightarrow &  &  &  &  &  &  &  &  &  &                                               &                &            &                &     \\
\lstick{\ket{\Psi_{2^i,k \Mod{2^i}}}}         & \gate{U_k} & \qw &             &  &  &  &  &  &  &  &  &  & \lstick{\ket{\Psi_{2^i,k \Mod{2^i}}}}         & \qswap \qwx[8] & \qw        & \qswap \qwx[8] & \qw \\
\lstick{\vdots}                               &            &     &             &  &  &  &  &  &  &  &  &  & \lstick{\vdots}                               &                &            &                &     \\
                                              &            &     &             &  &  &  &  &  &  &  &  &  &                                               &                &            &                &     \\
\lstick{\ket{\Psi_{2^{\hat{i}},2^{\hat{i}}}}} & \qw        & \qw &             &  &  &  &  &  &  &  &  &  & \lstick{\ket{\Psi_{2^{\hat{i}},2^{\hat{i}}}}} & \qw            & \qw        & \qw            & \qw \\
                                              &            &     &             &  &  &  &  &  &  &  &  &  &                                               &                &            &                &     \\
                                              &            &     &             &  &  &  &  &  &  &  &  &  & \lstick{\ket{a_{1}}}                          & \qw            & \qw        & \qw            & \qw \\
                                              &            &     &             &  &  &  &  &  &  &  &  &  & \lstick{\vdots}                               &                &            &                &     \\
                                              &            &     &             &  &  &  &  &  &  &  &  &  &                                               &                &            &                &     \\
                                              &            &     &             &  &  &  &  &  &  &  &  &  & \lstick{\ket{a_{k}}}                          & \qswap         & \gate{U_k} & \qswap         & \qw \\
                                              &            &     &             &  &  &  &  &  &  &  &  &  & \lstick{\vdots}                               &                &            &                &     \\
                                              &            &     &             &  &  &  &  &  &  &  &  &  &                                               &                &            &                &     \\
                                              &            &     &             &  &  &  &  &  &  &  &  &  & \lstick{\ket{a_{n-1}}}                        & \qw            & \qw        & \qw            & \qw
}

==> uselesscomments.tex <==

\begin{comment}
step by step
\begin{align*}
    \Pi_{xk}&=[U_{\sigma_x(n-1)}...U_{\sigma_x((k+1)\cdot \hat{n})}]\ 
    (U_{\sigma_x((k+1)\cdot \hat{n}-1)}...U_{\sigma_x(k\cdot \hat{n})})\ 
    [U_{\sigma_x(k\cdot \hat{n}-1)}...U_{\sigma_x(0)}]\\
    &=\alpha_{xk1}\cdot[U_{\sigma_x(n-1)}...U_{\sigma_x((k+1)\cdot \hat{n})}]\ 
    [U_{\sigma_x((k+1)\cdot \hat{n}-1)}...U_{\sigma_x(k\cdot \hat{n})}]\ 
    [U_{\sigma_x(k\cdot \hat{n}-1)}...U_{\sigma_x(0)}]\\
    &=\alpha_{xk1}\cdot\alpha_{xk2}\cdot[U_{\sigma_x(n-1)}...U_{\sigma_x(k\cdot \hat{n})}]\ 
    [U_{\sigma_x(k\cdot \hat{n}-1)}...U_{\sigma_x(0)}]\\
    &=\alpha_{xk1}\cdot\alpha_{xk2}\cdot\alpha_{xk3}\cdot[U_{\sigma_x(n-1)}...U_{\sigma_x(0)}]\\
    &=\alpha_{xk1}\cdot\alpha_{xk2}\cdot\alpha_{xk3}\cdot\Pi_0
\end{align*}
With:
\begin{align}
    (U_{\sigma_x((k+1)\cdot \hat{n}-1)}...U_{\sigma_x(k\cdot \hat{n})})&=\prod_{\substack{(k+1)\cdot \hat{n}> i>j\geq k\cdot \hat{n},\\\text{with } \sigma_x(i)<\sigma_x(j) }}\alpha_{\sigma_x(i)\sigma_x(j)}\cdot [U_{\sigma_x((k+1)\cdot \hat{n}-1)}...U_{\sigma_x(k\cdot \hat{n})}]\\
    [U_{\sigma_x(n-1)}...U_{\sigma_x((k+1)\cdot \hat{n})}]\ 
    [U_{\sigma_x((k+1)\cdot \hat{n}-1)}...U_{\sigma_x(k\cdot \hat{n})}]&=\prod_{\substack{n-1\geq i\geq (k+1)\cdot \hat{n}>j\geq k\cdot \hat{n},\\\text{with } \sigma_x(i)<\sigma_x(j) }}\alpha_{\sigma_x(i)\sigma_x(j)}\cdot [U_{\sigma_x(n-1)}...U_{\sigma_x(k\cdot \hat{n})}]
\end{align}
\begin{align*}
    \alpha_{xk1}&=\prod_{\substack{(k+1)\cdot \hat{n}> i>j\geq k\cdot \hat{n},\\\text{with } \sigma_x(i)<\sigma_x(j) }}\alpha_{\sigma_x(i)\sigma_x(j)}\\
    \alpha_{xk2}&=\prod_{\substack{n-1\geq i\geq (k+1)\cdot \hat{n}>j\geq k\cdot \hat{n},\\\text{with } \sigma_x(i)<\sigma_x(j) }}\alpha_{\sigma_x(i)\sigma_x(j)}\\
    \alpha_{xk3}&=\prod_{\substack{n-1\geq i\geq k\cdot \hat{n}>j\geq 0,\\\text{with } \sigma_x(i)<\sigma_x(j) }}\alpha_{\sigma_x(i)\sigma_x(j)}
\end{align*}
\begin{align*}
    \alpha_{xk1}\cdot \alpha_{xk2}&=\prod_{\substack{(k+1)\cdot \hat{n}>j\geq k\cdot \hat{n} \text{ and } n-1\geq i>j,\\\text{with } \sigma_x(i)<\sigma_x(j) }}\alpha_{\sigma_x(i)\sigma_x(j)}
\end{align*}
\end{comment}


\begin{comment}
\begin{align*}
    &\ket{00000000}\otimes ECA\ket{\Psi_1}\otimes DBA\ket{\Psi_2}\otimes EA\ket{\Psi_3}\otimes DA\ket{\Psi_4}\otimes CA\ket{\Psi_5}\otimes EA\ket{\Psi_6}+...\\
    &+\ket{10111100}\otimes CAE\ket{\Psi_1}\otimes ABD\ket{\Psi_2}\otimes AE\ket{\Psi_3}\otimes AE\ket{\Psi_4}\otimes CA\ket{\Psi_5}\otimes EA\ket{\Psi_6}+...\\
    =&(\ket{00000000}+...+\omega^{91 y}\ket{10111100}+...)\\
    &\otimes ECA\ket{\Psi_1}\otimes DBA\ket{\Psi_2}\otimes EA\ket{\Psi_3}\otimes DA\ket{\Psi_4}\otimes CA\ket{\Psi_5}\otimes EA\ket{\Psi_6}
\end{align*}

$$\Qcircuit @C=0.3em @R=0.3em {
\lstick{\ket{b}...} & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \text{...} &  & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw \\
\lstick{\ket{\Psi_{1}}...} & \qw & \multigate{11}{\mathcal{S}} & \qw &\gate{A} &\qw& \multigate{11}{\mathcal{S}} & \qw &\gate{B} &\qw& \multigate{11}{\mathcal{S}} & \qw &\gate{C} &\qw& \multigate{11}{\mathcal{S}} &\qw & \text{...} && \multigate{11}{\mathcal{S}} & \qw &\gate{H} &\qw& \multigate{11}{\mathcal{S}} & \qw &\gate{I} &\qw& \multigate{11}{\mathcal{S}} & \qw &\qw &\qw & \multigate{11}{\mathcal{S}} & \qw\\
\lstick{\ket{\Psi_{2}}...} & \qw & \ghost{\mathcal{S}}& \qw &\qw&\qw& \ghost{\mathcal{S}}& \qw &\gate{A}&\qw& \ghost{\mathcal{S}}& \qw &\gate{B}&\qw& \ghost{\mathcal{S}} & \qw &\text{...}      && \ghost{\mathcal{S}}& \qw &\gate{G}      &\qw& \ghost{\mathcal{S}}        & \qw &\gate{H}      &\qw& \ghost{\mathcal{S}} & \qw&\gate{I} &\qw & \ghost{\mathcal{S}} & \qw\\
\lstick{\ket{\Psi_{3}}...} & \qw & \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\text{...}      && \ghost{\mathcal{S}}        & \qw &\qw     &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw &\qw & \ghost{\mathcal{S}} & \qw\\
\lstick{\ket{a_A}...} & \qw & \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\text{...}      && \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw &\qw & \ghost{\mathcal{S}} & \qw\\
\lstick{\ket{a_B}...} & \qw & \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\text{...}      && \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw &\qw & \ghost{\mathcal{S}} & \qw\\
\vdots &&&&\vdots&&&&\vdots&&&&\vdots&&&& &&&&\vdots&&&&\vdots&&&&\vdots&&&&\\
\lstick{\ket{a_I}...} & \qw & \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\text{...}      && \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw &\qw & \ghost{\mathcal{S}} & \qw\\
\lstick{\ket{\Phi_{2}}...} & \qw & \ghost{\mathcal{S}} & \qw &\gate{I} &\qw& \ghost{\mathcal{S}} & \qw &\gate{H} &\qw& \ghost{\mathcal{S}} & \qw &\gate{G} &\qw& \ghost{\mathcal{S}} &\qw & \text{...} && \ghost{\mathcal{S}} & \qw &\gate{B} &\qw& \ghost{\mathcal{S}} & \qw &\gate{A} &\qw& \ghost{\mathcal{S}} & \qw &\qw &\qw & \ghost{\mathcal{S}} & \qw\\
\lstick{\ket{\Phi_{3}}...} & \qw & \ghost{\mathcal{S}}& \qw &\qw&\qw& \ghost{\mathcal{S}}& \qw &\gate{I}&\qw& \ghost{\mathcal{S}}& \qw &\gate{H}&\qw& \ghost{\mathcal{S}} & \qw &\text{...}      && \ghost{\mathcal{S}}& \qw &\gate{C}      &\qw& \ghost{\mathcal{S}}        & \qw &\gate{B}      &\qw& \ghost{\mathcal{S}} & \qw&\gate{A} &\qw & \ghost{\mathcal{S}} & \qw\\
\lstick{\ket{a^\prime_A}...} & \qw & \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\text{...}      && \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw &\qw & \ghost{\mathcal{S}} & \qw\\
\vdots &&&&\vdots&&&&\vdots&&&&\vdots&&&& &&&&\vdots&&&&\vdots&&&&\vdots&&&&\\
\lstick{\ket{a^\prime_I}...} & \qw & \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\text{...}      && \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw      &\qw& \ghost{\mathcal{S}}        & \qw &\qw &\qw & \ghost{\mathcal{S}} & \qw
}$$
\end{comment}

\begin{comment}
$$\Qcircuit @C=0.3em @R=0.3em {
&&&&&&&&&&&&\mbox{\textbf{repeated for every $k\in\{1,...,\hat{k}-1\}$}}&\\
\lstick{\ket{C}...} & \qw & \ctrl{1} &  \qw & \qw & \qw & \ctrl{1} & \ctrl{1} & \qw & \qw & \qw & \ctrl{1}  & \qw & \text{...} && \ctrl{1}  & \qw & \qw & \qw  & \ctrl{1}& \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw &...\\
\lstick{\ket{\Psi_{0}}...} & \qw & \multigate{11}{\mathcal{S}} & \qw &\qw &\qw& \multigate{11}{\mathcal{S}^{-1}} & \multigate{11}{\mathcal{S}} & \qw &\qw &\qw& \multigate{11}{\mathcal{S}^{-1}} & \qw &\text{...} && \multigate{11}{\mathcal{S}} &\qw & \qw& \qw & \multigate{11}{\mathcal{S}^{-1}} & \multigate{11}{\mathcal{S}} & \qw &\qw &\qw& \multigate{11}{\mathcal{S}^{-1}} & \qw&...\\
\vdots&&&&\vdots&&&&&\vdots&&&&\vdots&&&&\vdots&&&&&\vdots&&&&\vdots\\
\lstick{\ket{\Psi_{k}}...} & \qw & \ghost{\mathcal{S}}& \qw &\gate{U_{0}}&\qw& \ghost{\mathcal{S}^{-1}}& \ghost{\mathcal{S}}& \qw &\gate{U_{1}}&\qw& \ghost{\mathcal{S}^{-1}}& \qw &\text{...}      && \ghost{\mathcal{S}}& \qw &\gate{U_{n-2}}      &\qw& \ghost{\mathcal{S}^{-1}}        & \ghost{\mathcal{S}}& \qw &\gate{U_{n-1}}      &\qw& \ghost{\mathcal{S}^{-1}}        & \qw&...\\
\vdots&&&&\vdots&&&&&\vdots&&&&\vdots&&&&\vdots&&&&&\vdots&&&&\vdots\\
\lstick{\ket{\Psi_{\hat{k}-1}}...} & \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \ghost{\mathcal{S}}& \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \qw &\text{...} && \ghost{\mathcal{S}} &\qw & \qw& \qw & \ghost{\mathcal{S}^{-1}} & \ghost{\mathcal{S}}& \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \qw&...\\
\lstick{\ket{\Phi_{0}}...} & \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \ghost{\mathcal{S}}& \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \qw &\text{...} && \ghost{\mathcal{S}} &\qw & \qw& \qw & \ghost{\mathcal{S}^{-1}} & \ghost{\mathcal{S}}& \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \qw&...\\
\vdots&&&&\vdots&&&&&\vdots&&&&\vdots &&&&\vdots&&&&&\vdots&&&&\vdots\\
\lstick{\ket{\Phi_{\hat{k}-1}}...} & \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \ghost{\mathcal{S}}& \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \qw &\text{...} && \ghost{\mathcal{S}} &\qw & \qw& \qw & \ghost{\mathcal{S}^{-1}} & \ghost{\mathcal{S}}& \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \qw&...\\
\lstick{\ket{a_0}...} & \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \ghost{\mathcal{S}}& \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \qw &\text{...} && \ghost{\mathcal{S}} &\qw & \qw& \qw & \ghost{\mathcal{S}^{-1}} & \ghost{\mathcal{S}}& \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \qw&...\\
\lstick{\ket{a_1}...} & \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \ghost{\mathcal{S}}& \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \qw &\text{...} && \ghost{\mathcal{S}} &\qw & \qw& \qw & \ghost{\mathcal{S}^{-1}} & \ghost{\mathcal{S}}& \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \qw&...\\
\vdots&&&&\vdots&&&&&\vdots&&&&\vdots&&&&\vdots&&&&&\vdots&&&&\vdots\\
\lstick{\ket{a_{n-1}}...} & \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \ghost{\mathcal{S}}& \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \qw &\text{...} && \ghost{\mathcal{S}} &\qw & \qw& \qw & \ghost{\mathcal{S}^{-1}} & \ghost{\mathcal{S}}& \qw &\qw &\qw& \ghost{\mathcal{S}^{-1}} & \qw&...\gategroup{2}{3}{14}{25}{.8em}{--}
}$$
$$\Qcircuit @C=0.3em @R=0.3em {
&&&&&&&&&&&&\mbox{\textbf{repeated for every $k\in\{1,...,\hat{k}-1\}$}}&\\
\lstick{\ket{C}...} & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \text{...} && \ctrl{1} & \qw & \qw & \qw  & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw &...\\
\lstick{\ket{\Psi_{0}}...} & \qw & \multigate{11}{\mathcal{S}} & \qw &\qw &\qw& \multigate{11}{\mathcal{S}} & \qw &\qw &\qw& \multigate{11}{\mathcal{S}} & \qw &\text{...} && \multigate{11}{\mathcal{S}} &\qw & \qw& \qw & \multigate{11}{\mathcal{S}} & \qw &\qw &\qw& \multigate{11}{\mathcal{S}} & \qw&...\\
\vdots&&&&\vdots&&&&\vdots&&&&\vdots&&&&\vdots&&&&\vdots&&&&\vdots\\
\lstick{\ket{\Psi_{k}}...} & \qw & \ghost{\mathcal{S}}& \qw &\gate{U_{0}}&\qw& \ghost{\mathcal{S}}& \qw &\gate{U_{1}}&\qw& \ghost{\mathcal{S}}& \qw &\text{...}      && \ghost{\mathcal{S}}& \qw &\gate{U_{n-2}}      &\qw& \ghost{\mathcal{S}}        & \qw &\gate{U_{n-1}}      &\qw& \ghost{\mathcal{S}}        & \qw&...\\
\vdots&&&&\vdots&&&&\vdots&&&&\vdots&&&&\vdots&&&&\vdots&&&&\vdots\\
\lstick{\ket{\Psi_{\hat{k}-1}}...} & \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw &\text{...} && \ghost{\mathcal{S}} &\qw & \qw& \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw&...\\
\lstick{\ket{\Phi_{0}}...} & \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw &\text{...} && \ghost{\mathcal{S}} &\qw & \qw& \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw&...\\
\vdots&&&&\vdots&&&&\vdots&&&&\vdots &&&&\vdots&&&&\vdots&&&&\vdots\\
\lstick{\ket{\Phi_{\hat{k}-1}}...} & \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw &\text{...} && \ghost{\mathcal{S}} &\qw & \qw& \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw&...\\
\lstick{\ket{a_0}...} & \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw &\text{...} && \ghost{\mathcal{S}} &\qw & \qw& \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw&...\\
\lstick{\ket{a_1}...} & \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw &\text{...} && \ghost{\mathcal{S}} &\qw & \qw& \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw&...\\
\vdots&&&&\vdots&&&&\vdots&&&&\vdots&&&&\vdots&&&&\vdots&&&&\vdots\\
\lstick{\ket{a_{n-1}}...} & \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw &\text{...} && \ghost{\mathcal{S}} &\qw & \qw& \qw & \ghost{\mathcal{S}} & \qw &\qw &\qw& \ghost{\mathcal{S}} & \qw&...\gategroup{2}{3}{14}{23}{.8em}{--}
}$$

\end{comment}

\begin{align}
    &\sum_{\substack{x_{ijk}\\ \text{with }i\neq j\neq k}}\ket{x_{ijk}}\otimes \ket{\Psi_t}\otimes \ket{a_0}\otimes \ket{a_1}\\
    &\rightarrow \sum_{\substack{x_{ijk}\\ \text{with }i\neq j\neq k}}\ket{x_{ijk}}\otimes U_iU_jU_k \ket{\Psi_t}\otimes \ket{a_0}\otimes \ket{a_1}\\
    &=\sum_{\substack{x_{ijk}\\ \text{with }i\neq j\neq k}}\omega^{x_{ijk}\cdot y}\ket{x_{ijk}}\otimes U_iU_jU_k \ket{\Psi_t}\otimes \ket{a_0}\otimes \ket{a_1}\\
\end{align}


It is true that the algorithm with six queries presented in ... can solve this FPP since there only the fact that there are pairwise commutation relations is important (the switch and the simulation thereof can solve it clearly as well, one just has to match the label to the corresponding permutation). 
But the FPP with this labeling cannot be solved with the algorithm presented in this section, since here we make explicit use of the pairwise commutation relations that are induced by the factoradic labeling: $U_jU_k=\omega^{k!\cdot y}\cdot U_kU_j$ ($j<k$).

\begin{comment}
Note that this property is equivalent to the original promise (the other direction follows from direct computation, be careful!):
\begin{align}
    \forall j,k: U_jU_k=\omega^{(x_1-x_2)\cdot y}\cdot U_kU_j \Leftrightarrow \forall x: \Pi_x=\omega^{x\cdot y}\cdot \Pi_0
\end{align}
\end{comment}
In the next Section, we show how to use this property to solve a certain FPP with a causal algorithm that uses $O(n\log{n})$ queries. In Section 4, we will show that there is a causal algorithm that can solve every FPP with $O(n\sqrt{n})$ queries.
%unten stehendes comment; mehr auf labeling eingehen?

\begin{comment}
We  all permutation relations can be reduced to pairwise permutation relations.

\begin{align}
    \left(\sum_{x=0}^{n!-1}\omega^{x\cdot y}\ket{x}\right)\otimes ...
\end{align}
in the control system after applying a quantum circuit. If the control system factors out in this state, the task is solved by measuring the system in the Fourier basis. 
\end{comment}

%Using the only known precise labeling of permutations (up to our knowledge), namely the one given in Appendix A of \cite{1}, we show in the next Section that this property can be used to solve the task with a causal algorithm that uses $O(n\log{n})$ queries. 


%\subsection{Pairwise commutation relations}
\begin{comment}
For this note that every Fourier Promise Problem imply pairwise commutation relations in the sense that for every pair of unitaries $U_j$ and $U_k$ there is $\alpha_{jk}\in \mathbb{C}$ (the dependence of $\alpha_{jk}$ on $y$ is implicit) such that (assume without loss of generality $j<k$)
\begin{align*}
    U_jU_k=\alpha_{jk}\cdot U_kU_j.
\end{align*}
\end{comment}
